Scattering diagrams in mirror symmetry

Since the pioneering work of Kontsevich and Soibelman [51], scattering diagrams have started playing an important role in mirror symmetry, in particular in the study of the reconstruction problem. This paper aims at introducing the main ideas on the subject describing the role of scattering diagrams in relation to the SYZ conjecture and the HMS conjecture.

==> localcommands.tex <==
\newcommand*{\orcid}{}


==> localpackages.tex <==
% add all extra packages you need to load to this file  
\usepackage{tabularx} 

% \usepackage{langsci-branding}
\usepackage{langsci-optional}
 

